Improving Text-based Early Prediction by Distillation from Privileged Time-Series Text

Modeling text-based time-series to make prediction about a future event or outcome is an important task with a wide range of applications. The standard approach is to train and test the model using the same input window, but this approach neglects the data collected in longer input windows between the prediction time and the final outcome, which are often available during training. In this study, we propose to treat this neglected text as privileged information available during training to enhance early prediction modeling through knowledge distillation, presented as Learning using Privileged tIme-sEries Text (LuPIET). We evaluate the method on clinical and social media text, with four clinical prediction tasks based on clinical notes and two mental health prediction tasks based on social media posts. Our results show LuPIET is effective in enhancing text-based early predictions, though one may need to consider choosing the appropriate text representation and windows for privileged text to achieve optimal performance. Compared to two other methods using transfer learning and mixed training, LuPIET offers more stable improvements over the baseline, standard training. As far as we are concerned, this is the first study to examine learning using privileged information for time-series in the NLP context.

==> sections/archive_result.tex <==
\begin{table*}[h!]
\centering
\small
% \hspace*{-2.4cm}

\resizebox{\linewidth}{!}{%
\begin{tabular}{|l|c c|c c|c c|c c|}
\hline

\multirow{2}{*}{}    & \multicolumn{2}{c|}{Mort hosp} & \multicolumn{2}{c|}{Mort ICU} & \multicolumn{2}{c|}{LOS$>$3days} & \multicolumn{2}{c|}{DRG} \\ \cline{2-9} 
& AUROC  & AUPR   & AUROC   & AUPR & AUROC   & AUPR &  Acc   & MacroF1   \\ \hline 


% content


\textbf{\textit{Baseline}}
& & & & & & & & \\
1d 

& \makecell{0.844 \\ (0.0058)} & \makecell{0.417 \\ (0.0122)} & \makecell{0.860 \\ (0.0049)} & \makecell{0.369 \\ (0.0172)} & \makecell{0.695 \\ (0.0059)} & \makecell{0.629 \\ (0.0061)} & \makecell{0.228 \\ (0.0057)} & \makecell{0.056 \\ (0.0043)}\\

\hline

\textbf{\textit{Mix train}}
& & & & & & & & \\
1d + 3d + 7d

 & \makecell{0.838 \\ (0.0019)} & \makecell{0.416 \\ (0.0113)} & \textbf{\makecell{0.866 \\ (0.0055)}} & \textit{\makecell{0.382 \\ (0.0125)}} & \makecell{0.671 \\ (0.0035)} & \makecell{0.605 \\ (0.0066)} & \makecell{0.236 \\ (0.0073)} & \makecell{0.061 \\ (0.0043)}\\

\hline

\textbf{\textit{Transfer}}
& & & & & & & & \\

3d -$>$ 1d
 & \textbf{\makecell{0.853 \\ (0.0038)}} & \textbf{\makecell{0.439 \\ (0.0080)}} & \makecell{0.862 \\ (0.0069)} & \textbf{\makecell{0.384 \\ (0.0093)}} & \makecell{0.688 \\ (0.0022)} & \makecell{0.615 \\ (0.0044)} & \makecell{0.232 \\ (0.0067)} & \makecell{0.059 \\ (0.0043)}\\

7d -$>$ 1d
 & \makecell{0.833 \\ (0.0037)} & \makecell{0.415 \\ (0.0086)} & \makecell{0.861 \\ (0.0065)} & \makecell{0.371 \\ (0.0123)} & \makecell{0.686 \\ (0.0056)} & \makecell{0.623 \\ (0.0057)} & \makecell{0.230 \\ (0.0070)} & \makecell{0.064 \\ (0.0039)}\\

7d -$>$ 3d -$>$ 1d
 & \makecell{0.829 \\ (0.0073)} & \makecell{0.405 \\ (0.0108)} & \makecell{0.861 \\ (0.0080)} & \makecell{0.362 \\ (0.0147)} & \makecell{0.688 \\ (0.0029)} & \makecell{0.621 \\ (0.0022)} & \makecell{0.232 \\ (0.0052)} & \textbf{\makecell{0.066 \\ (0.0049)}}\\

\hline

\textbf{\textit{Temporal KD}}
& & & & & & & & \\

Teacher 3d
 & \makecell{0.850 \\ (0.0040)} & \makecell{0.428 \\ (0.0108)} & \makecell{0.861 \\ (0.0060)} & \makecell{0.362 \\ (0.0178)} & \makecell{0.696 \\ (0.0034)} & \makecell{0.631 \\ (0.0054)} & \textbf{\makecell{0.238 \\ (0.0063)}} & \makecell{0.056 \\ (0.0055)}\\

Teacher 7d
 & \makecell{0.851 \\ (0.0033)} & \makecell{0.430 \\ (0.0125)} & \makecell{0.860 \\ (0.0046)} & \makecell{0.370 \\ (0.0168)} & \textbf{\makecell{0.698 \\ (0.0027)}} & \textbf{\makecell{0.635 \\ (0.0039)}} & \makecell{0.237 \\ (0.0042)} & \makecell{0.057 \\ (0.0029)}\\

\hline

% content ends

\end{tabular}}
    \caption{Results of different methods.}
    \label{tab:res1}
\end{table*}



On LSTM with document embedding, transferring learning model, which pre-trains on the late data first and then fine-tunes on early data, offers overall best results. However, we can also observe that the transfer learning approach sometimes depends on the specific late windows for certain tasks. For example, in-hospital mortality prediction actually drops when transferring from 7-day data, and prolonged LOS prediction also suffers from this transfer learning. Similarly, mixed training can improve performance in certain cases, such as on in-ICU mortality prediction, but could harm other tasks. In contrast, we do not see temporal knowledge distillation dampen the baseline performance in any task, though its improvement over baseline may be limited with LSTM plus document embedding. 

\begin{table*}[!h]
\centering

\resizebox{\linewidth}{!}{%
\begin{tabular}{|l|c c|c c|c c|c c|}
\hline

\multirow{2}{*}{}    & \multicolumn{2}{c|}{Mort hosp} & \multicolumn{2}{c|}{Mort ICU} & \multicolumn{2}{c|}{LOS$>$3days} & \multicolumn{2}{c|}{DRG} \\ \cline{2-9} 
& AUROC  & AUPR   & AUROC   & AUPR & AUROC   & AUPR &  Acc   & MacroF1   \\ \hline 


% content

\textbf{\textit{Baseline}}
& & & & & & & & \\
1d 
 & \makecell{0.867 \\ (0.0032)} & \makecell{0.474 \\ (0.0151)} & \makecell{0.862 \\ (0.0110)} & \makecell{0.373 \\ (0.0252)} & \makecell{0.690 \\ (0.0034)} & \makecell{0.625 \\ (0.0047)} & \makecell{0.282 \\ (0.0058)} & \makecell{0.105 \\ (0.0106)}\\

\hline
\textbf{\textit{Mix train}}
& & & & & & & & \\
1d + 3d + 7d

 & \makecell{0.866 \\ (0.0031)} & \makecell{0.490 \\ (0.0031)} & \makecell{0.860 \\ (0.0079)} & \makecell{0.398 \\ (0.0077)} & \makecell{0.642 \\ (0.0037)} & \makecell{0.561 \\ (0.0057)} & \makecell{0.298 \\ (0.0025) } & \textbf{\makecell{0.140 \\ (0.0081)}} \\

\hline
\textbf{\textit{Transfer}}
& & & & & & & & \\

3d -$>$ 1d
 & \makecell{0.863 \\ (0.0026)} & \makecell{0.466 \\ (0.0063)} & \makecell{0.866 \\ (0.0060)} & \makecell{0.381 \\ (0.0231)} & \makecell{0.695 \\ (0.0036)} & \makecell{0.612 \\ (0.0049)} & \makecell{0.293 \\ (0.0033)} & \makecell{0.134 \\ (0.0059)}\\

7d -$>$ 1d
 & \makecell{0.865 \\ (0.0040)} & \makecell{0.482 \\ (0.0073)} & \makecell{0.860 \\ (0.0051)} & \makecell{0.379 \\ (0.0089)} & \makecell{0.691 \\ (0.0046)} & \makecell{0.616 \\ (0.0068)} & \makecell{0.284 \\ (0.0027)} & \makecell{0.113 \\ (0.0072)}\\
7d -$>$ 3d -$>$ 1d
 & \makecell{0.864 \\ (0.0040)} & \makecell{0.482 \\ (0.0110)} & \makecell{0.855 \\ (0.0073)} & \makecell{0.374 \\ (0.0098)} & \makecell{0.683 \\ (0.0031)} & \makecell{0.606 \\ (0.0054)} & \makecell{0.285 \\ (0.0093)} & \makecell{0.112 \\ (0.0081)}\\
dsumm -$>$ 1d
 & \makecell{0.863 \\ (0.0052)} & \makecell{0.480 \\ (0.0155)} & \makecell{0.865 \\ (0.0097)} & \makecell{0.399 \\ (0.0157)} & \textbf{\makecell{0.704 \\ (0.0028)}} & \textbf{\makecell{0.639 \\ (0.0060)}} & \textbf{\makecell{0.304 \\ (0.0064)}} & \makecell{0.139 \\ (0.0081)}\\
dsumm -$>$ 7d -$>$ 1d
 & \makecell{0.864 \\ (0.0033)} & \makecell{0.485 \\ (0.0133)} & \makecell{0.855 \\ (0.0102)} & \makecell{0.387 \\ (0.0209)} & \makecell{0.691 \\ (0.0043)} & \makecell{0.615 \\ (0.0073)} & \makecell{0.302 \\ (0.0044)} & \makecell{0.137 \\ (0.0050)}\\
dsumm -$>$ 7d -$>$ 3d -$>$ 1d
 & \makecell{0.860 \\ (0.0069)} & \makecell{0.482 \\ (0.0091)} & \makecell{0.842 \\ (0.0083)} & \makecell{0.359 \\ (0.0182)} & \makecell{0.686 \\ (0.0038)} & \makecell{0.606 \\ (0.0076)} & \textbf{\makecell{0.304 \\ (0.0035)}} & \makecell{0.138 \\ (0.0026)}\\

\hline
\textbf{\textit{Temporal KD}}
& & & & & & & & \\

Teacher 3d
 & \makecell{0.876 \\ (0.0027)} & \makecell{0.491 \\ (0.0039)} & \textbf{\makecell{0.880 \\ (0.0020)}} & \textbf{\makecell{0.429 \\ (0.0092)}} & \makecell{0.693 \\ (0.0042)} & \makecell{0.626 \\ (0.0058)} & \makecell{0.287 \\ (0.0068)} & \makecell{0.116 \\ (0.0067)}\\
Teacher 7d
 & \textbf{\makecell{0.879 \\ (0.0029)}} & \textbf{\makecell{0.501 \\ (0.0093)}} & \makecell{0.880 \\ (0.0024)} & \makecell{0.413 \\ (0.0076)} & \makecell{0.692 \\ (0.0035)} & \makecell{0.627 \\ (0.0041)} & \makecell{0.290 \\ (0.0097)} & \makecell{0.115 \\ (0.0130)}\\
Teacher dsumm
 & \makecell{0.859 \\ (0.0191)} & \makecell{0.457 \\ (0.0502)} & \makecell{0.863 \\ (0.0117)} & \makecell{0.382 \\ (0.0238)} & \makecell{0.695 \\ (0.0029)} & \makecell{0.629 \\ (0.0041)} & \makecell{0.302 \\ (0.0081)} & \makecell{0.130 \\ (0.0101)}\\
 
\hline

% content ends

\end{tabular}}
    \caption{Results of different methods.}
    \label{tab:res1}
\end{table*}



When applying MultiResCNN with word embedding to the same cohorts on the same tasks, we see similar overall performance trends and some different phenomena. In general, transfer learning can still offer competitive results and sometimes the best results compared to other methods. Similarly, mixed training also improves certain tasks significantly, like DRG. However, again, these two approaches may harm the results on some other tasks compared to baseline, and the benefit of transfer learning is sensitive to the selection of the pre-training window. On the other hand, temporal KD improves over baseline consistently (except distilling discharge summary for mortality prediction, in which cases the teacher models perform worse). Unlike the document embedding model, MultiResCNN at the word level seems to benefit more from temporal KD, as we see much better mortality predictions scores than others. This may indicate that the proper training of KD exploits the nuances in the data so it would benefit more when modeling at a finer granularity. 
